Sequential sampling of junction trees for decomposable graphs

The junction-tree representation provides an attractive structural property for organizing a decomposable graph. In this study, we present two novel stochastic algorithms, which we call the junction-tree expander and junction-tree collapser for sequential sampling of junction trees for decomposable graphs. We show that recursive application of the junction-tree expander, expanding incrementally the underlying graph with one vertex at a time, has full support on the space of junction trees with any given number of underlying vertices. On the other hand, the junction-tree collapser provides a complementary operation for removing vertices in the underlying decomposable graph of a junction tree, while maintaining the junction tree property. A direct application of our suggested algorithms is demonstrated in a sequential-Monte-Carlo setting designed for sampling from distributions on spaces of decomposable graphs. Numerical studies illustrate the utility of the proposed algorithms for combinatorial computations on decomposable graphs and junction trees. All the methods proposed in the paper are implemented in the Python library trilearn.

==> ex_cta.tex <==
% -*- root: opr2018.tex -*-
\begin{myex} \label{ex:cta}
    Figure~\ref{fig:ct} shows a junction tree (left panel) and a possible expanded version (right panel) where the subtree chosen in Step~1 contains the nodes $(\jtnode[i])_{i=1}^8$.
    This subtree is then replaced by the one containing the new nodes $(\jtnewnode{i})_{i=1}^8$ and having isomorphic structure.
    Those of the old nodes that were not engulfed by a new node are connected to the new nodes, giving the expanded tree the appearance of a Christmas tree.
    \begin{figure}
    \centering
    \begin{subfigure}[b]{0.30\textwidth}

        \resizebox{5cm}{5cm}{
            \input{figures/tikz/to_be_ct.tikz}
        }
        %\includegraphics[width=\textwidth]{figures/tikz/to_be_ct}
    \end{subfigure}
~\hspace{7mm}%
    \begin{subfigure}[b]{0.30\textwidth}
        \resizebox{5cm}{5cm}{
            \input{figures/tikz/ct.tikz}
        }
        %\includegraphics[width=\textwidth]{figures/tikz/ct}
    \end{subfigure}

    \caption{The junction tree in Example~\ref{ex:cta} (left panel) along with its expansion (right panel).} 
    \label{fig:ct}
\end{figure}
\end{myex}

==> intro-new.tex <==
\jimmy{At present, I don't think that we manage to explain the very knowledge gap that this paper is filling, and it will probably be quite hard for the reviewers to understand our contribution.}
Decomposable graphs and their junction-tree representations as auxiliary data structure have been used in various contexts; examples include computational geometry, large-scale estimation of random graph models with local dependence, statistical inference (such as sparse covariance- and concentration-matrix computation), contingency-table analysis, probabilistic graphical models, and message passing, see \emph{e.g.} \citep{lauritzen1996, pearl1997probabilistic, eppstein2009graph}.\jimmy{Add references for all these applications.} 
\felix{Punkt 1, tillämpningar}

In recent years, decomposable graphs have become an important and popular tool for representing dependence structures in probabilistic graphical models.
In the Bayesian setting, structure learning in such models amounts to calculating a posterior distribution defined on the space of decomposable graphs in order to gain understanding of the dependence structure underlying an observed data set. Due to the inherent complexity of distributions defined on such spaces, this has lead to an increasing interest in Monte Carlo methods for sampling-based approximations. 
%The complexity inherent in distributions defined on such spaces has lead to an increasing interest in Monte Carlo methods for sampling-based approximations. 
\felix{Punkt 2}
%Typical strategies are based on \emph{\mcmc}\, (\mcmcabbr)\, methods, especially variations of the \emph{Metropolis-Hastings algorithm} where, in each updating step, a new graph is proposed by subjecting the previous one to random edge perturbations, and the set of possible moves obtained by such single-edge perturbations defines a neighborhood in the decomposable-graph space from which new graphs can be sampled; see \emph{e.g}. \citep{frydenberg1989decomposition, Giudici01121999,Thomas:2009aa, Green01032013}.
Typical sampling strategies are based on \emph{\mcmc}\, (\mcmcabbr)\, methods, especially variations of the \emph{Metropolis-Hastings algorithm}, where new graphs are proposed by means of random single-edge perturbations, and the set of possible moves generated by subjecting a given graph to such perturbations defines a neighborhood in the decomposable-graph space; see \emph{e.g}. \citep{frydenberg1989decomposition, Giudici01121999,Thomas:2009aa, Green01032013}.
\felix{Punkt 3}
 However, since the only vertices that may be connected by an edge in a (connected) decomposable graph while maintaining decomposability are those that already have a neighbour in common and the removable edges are necessarily contained in exactly one clique, % may be connected by an edge, %of a decomposable graph is hard and since the number of edges grows very vast with the number of edges, such moves a are inherently local, 
 operations on the edge set are inherently local. As a consequence, an MCMC sampler based on such moves will most likely suffer from poor mixing. 
 
In the light of the previous, it is  desirable to explore alternative ways of simulating decomposable graphs. In the present paper we take a different approach which, instead of altering the edge set of a graph with a fixed set of vertices, builds new graphs incrementally, starting from the empty graph and adding vertices one by one. When applied to Monte Carlo simulation, this procedure allows for independent or weakly correlated samples.  
%In this paper we take a different approach to manipulating decomposable graphs, where instead of considering the node set as fixed while altering the edge set as in the above mentioned techniques, we consider alerting both the node set, which allows for sampling new graphs from scratch.
As we shall see, this approach can be designed more easily if one operates on the extended junction-tree space rather than directly on the space of decomposable graphs.
\felix{Punkt 4}

%A common issue for the above mentioned class of sampling techniques is that they suffer from poor mixing inherent by the local operations on the graph, which was the main motivation for the development of our work.
%More precisely, we present two novel stochastic operations on the junction-tree structure, specified by corresponding algorithms: 
In this paper we present two novel  stochastic algorithms operating on junction-tree structures:
the \emph{\jte}\, (\jteabbr, or the \emph{Christmas-tree algorithm}) and the \emph{\jtc} (\jtcabbr). % for sequentially sampling of junction trees.
More precisely, the \jteabbr\, (\jtcabbr) expands (collapses) a junction tree  \(\tree\) by randomly adding (removing) one vertex to (from) the underlying decomposable graph. 
At the highest level, the \jteabbr\, can be described in two main steps.
In the first step, the algorithm starts by drawing, at random, a subtree \(\tree'\) of the given tree \(\tree\) using a stochastic version of a depth-first tree-traversal. 
A new vertex  \(\gennodea\) is then connected to a random subset \jimmy{Subset? You mean subgraph?} of each of the cliques in \(\tree'\) to form a new subtree \(\tree''\),  which is isomorphic to \(\tree'\).
The second step amounts to drawing, for each clique in \(\tree''\), a neighboring clique not containing \(\gennodeb\), for which the clique is substituted while maintaining the junction tree property.\jimmy{Not completely clear to me what you mean by ``neighboring clique'' here, since $T''$ is in some sense an isolated tree after selection. As far as I remember, you expand the tree by connecting randomly the new cliques in $T''$ to the old ones in $T'$ when possible?} On the other hand, the \jtcabbr\, starts by selecting the unique subtree \(\tree''\) induced by a given vertex \(\gennodeb \).\jimmy{And?}
The two algorithms are complementary in the sense that the output obtained by subjecting a given tree $\tree$ to either the \jteabbr\, followed by the \jtcabbr, or, vice versa, the \jtcabbr\, followed by the \jteabbr, coincides with $\tree$ with positive probability. \felix{punkt 6}

In the \mcmcabbr\, approach taken by \citet{Green01032013}, a given probability mass function on the space of decomposable graphs is embedded into an extended version defined on the space of junction trees, where %; 
%more precisely, the probability assigned by the extended probability mass function to a given junction tree is set to be equal to the probability assigned by the original mass function to the tree's underlying graph divided by the number of junction-tree representations of that graph. As a consequence, 
the push-forward distribution of the extended distribution with respect to the underlying graph equals the given probability mass function on the decomposable-graph space. 
Thus, by running an \mcmcabbr\, sampler producing a trajectory of junction trees targeting the extended distribution, an \mcmcabbr\, trajectory targeting the original distribution is obtained as a by-product by simply extracting the underlying graphs of the trees in the former sequence.\felix{Punkt 5}
%Thus, by running a Monte Carlo sampler targeting the extended distribution, an Monte Carlo\, sampler targeting the original distribution is obtained as a by-product by simply extracting the underlying graphs of the trees in the former.\felix{Punkt 5}

%Further, we demonstrate that the algorithms constitute a key building block in the temporalisation technique of \cite{olsson2019}, be employed jointly to construct a \smc\, (\smcabbr) sampler for approximating arbitrary distributions over decomposable graphs.

By combining the junction tree extension from \citep{Green01032013}  with the temporalisation technique of \cite{olsson2019}, we demonstrate that the \jteabbr\, and \jtcabbr\, can be employed jointly to construct a \smc\, (\smcabbr) sampler for approximating arbitrary distributions over decomposable graphs.
%More specifically, the \jtcabbr\, is used to extend the junction tree distribution to a path space of junction trees of increasing dimension and the \jteabbr\, is used to generate proposals on this new space. 
As we shall see, the \jteabbr\, and \jtcabbr\, have two theoretical properties that are of crucial importance in this setting. %, in particular when applied for temporalisation. 
First, the transition probabilities of the induced Markov kernels are available in a closed form and can be computed efficiently; second, the \jteabbr\, algorithm is able to generate, with positive probability, when applied sequentially, all junction trees with a given number of vertices in its underlying graph.
%These properties seem much harder to obtain while maintaining the computational efficiency by working on directly on the space of decomposable graphs.
%From a structure learning perspective, I may seem more sensible to operate on the decomposable graph space directly, however while the latter property may be easy to achieve, the former one is more complex.
\felix{punkt 6 igen}

In the paper \citep{olsson2019}, we further incorporate the \smcabbr\, sampler in a \emph{particle Gibbs} algorithm, which builds completely upon the \jteabbr\, and \jtcabbr\, derived in the present paper, rendering \emph{global moves} on the decomposable graph space possible.

%which builds show that, by incorporating the \smcabbr\, sampler in a \emph{particle Gibbs} sampler, it is possible to provide \emph{global moves} on the decomposable graph space, in contrast to local edge perturbations.\jimmy{This is indeed the main motivation for doing what we are doing, and should be explained earlier. The logical flow is not super here.}

%Using the \smcabbr\, sampler
As a by-product of the \smcabbr\, approach presented in this paper, we are able to provide unbiased estimates of the numbers of decomposable graphs and junction trees with any given number of vertices. 
This importance-sampling approach to the combinatorics of decomposable graphs and junction trees is the first of its kind. \citet{countchordal} provides a closed-form expression for the number of decomposable graphs; however, calculations are tractable only for a very limited number of vertices. Up to our knowledge, there is no closed-form expression for the number of junction trees.\jimmy{I think that this application gets too much space here, since this implies again a large risk that the referees consider this paper too closely related to our companion paper.}
\felix{punkt 8}



%As a by-product of 
The \jteabbr\, is related to other existing approaches of generating junction trees. For instance, the algorithm for generation of junction trees presented in \citep{randchord} has similarities to ours in the sense that it incrementally expands the underlying graph in each step of the algorithm.
However, unlike our proposed \jteabbr, this algorithm is restricted to connected decomposable graphs and transition probabilities are not directly provided. 
%Further pertinent approaches include \emph{e.g.} \citep{stingo2015efficient}, where focus is on Gaussian graphical models. This restriction enables faster edge moves by dynamically updating the \emph{perfect sequence} of the cliques in the graph.\jimmy{Is this correct?} 
A completely different strategy for decomposable-graph sampling based on  {\it tree-dependent bipartiet graphs} is presented in \citet{elmasri2017decomposable, elmasri2017sub}.

%As a consequence the mixing properties of the resulting Markov chain are substantially improved.
%A thorough presentation of the \smcabbr\, algorithm together with the particle Gibbs sampling  scheme and further applications to  Bayesian structure learning  are presented in %the companion papers
%\citep{olsson2019, graphpred}. 
\felix{punkt 3}
%This subtree is then used as a template for the the structure of the subtree induced by the newly added vertex.
%\jimmy{Is this what we want to say?} 
%Said differently, since the \jteabbr\, and the \jtcabbr\, define Markov transition kernels between spaces of increasing and decreasing dimension, respectively, any product of the two kernels is positive on the diagonal. 
%Together, these two algorithms constitute a key building block for sampling from arbitrary graph and junction tree distributions using importance sampling.
% In this paper, we present a new algorithm which we call the \emph{\jte} or the  \emph{Christmas-tree algorithm}, for sequential sampling of junction trees.
% the algorithm we propose constructs incrementally junction trees by expanding randomly the underlying decomposable graph one vertex at a time.
%It differs substantially from the above-mentioned methods; rather than perturbing the edge set for a fixed set of vertices, the algorithm we propose constructs incrementally junction trees by expanding randomly the underlying decomposable graph one vertex at a time.
%The relevance of our suggested algorithm is justified from a Bayesian structure learning perspective, where it opens for a  novel, sequential approach for approximating \emph{weakly structural Markov} distributions \citep{green2017structural} over decomposable graphs based on \smc.
%In this setting the \jteabbr\, is employed as proposal kernel.
% sequential Monte Carlo (SMC) perspective for approximating \emph{weakly structural Markov} distributions over decomposable graphs; see \citep{green2017structural}, where the  \jteabbr\, is employed as proposal kernel.



% motivate why junction tree space


% By using the \jtc to create an extended target distribution, we demonstrate that the \jte can be used as a proposal kernel in a \smcabbr\, 
% sampling approach, we are able to provide unbiased estimates of normalising constants for weakly structural Markov laws.
%[Change: 
%\citet{olsson2019} show that, by incorporating the \smcabbr\, sampler in a \emph{particle Gibbs} sampler, it is possible to provide \emph{global moves} on the decomposable graph space, in contrast to local edge perturbations.
%As a consequence the mixing properties of the resulting Markov chain are substantially improved.
%A thorough presentation of the \smcabbr\, algorithm together with the particle Gibbs sampling  scheme and further applications to  Bayesian structure learning  are presented in %the companion papers
%\citep{olsson2019, graphpred}. ]

%[In the area of probabilistic graphical models, where graphs are used to describe the dependence structure of a multivariate probability distribution, a family of distributions which are Markov with respect to a decomposable graph is typically called a \emph{decomposable graphical model}, \cite{lauritzen1996}.
%Such models have a particularly appealing property that their distributions factorises as local distributions of the cliques and separators, which makes inference tasks in these models directly removes the problem of unknown normalising constants as is the problem with ordinary undirected graphs. 
%Recent advances \citep{bornn2011bayesian,green2017structural} shows that a certain class of graph distributions over \(\graphsp[\jtind]\), termed \emph{weakly structural Markov}, factorize over the cliques and separators in a similar manner as \emph{decomposable graphical models}.
%Such distributions arise naturally in Bayesian statistics and structure learning as %prior-, and due to their conjugate property, posterior graph distributions. 
%\cite{olsson2019} shows how the junction tree expander and collapser are used in a %particle Gibbs scheme tailored to approximate such distributions efficiently.]




The rest of this paper is structured as follows. Section \ref{sec:preliminaries} introduces some graph notation and a short background on decomposable graphs and the concept of junction trees. (For a more detailed presentation, the reader is referred to \emph{e.g.} \citep{ChordalGraphs} or \citep{lauritzen1996}.)
Section~\ref{sec:expanding_a_junction_tree} and Section~\ref{sub:rcta} present the \jteabbr\, and  the \jtcabbr\, along with their corresponding transition probabilities.
Section~\ref{sec:update_mu} provides a novel factorisation of the number of junction trees of a decomposable graph, and demonstrates its computational advantage.
The application of the \jteabbr\, and the \jtcabbr\, in framework of \smcabbr\, sampling scheme is found in Section~\ref{sec:smc} and 
Section~\ref{sec:simulations} contains our numerical study. 
%the first devoted to 
%Bayesian structure learning in Gaussian decomposable models and the second to decomposable graph combinatorics. 
%In the latter example, \smcabbr\, is used for providing unbiased estimates of the number of decomposable graphs of different number of vertices.
Appendix \ref{appendix:a} is devoted to detailed algorithm descriptions along with the proofs of lemmas and theorems stated in the paper, whereas Appendix \ref{appendix:b} provides an algorithm, originally presented in \citep{doi:10.1198/jcgs.2009.07129}, for randomly connecting a forest into a tree. 
\felix{9}
Finally, we remark that the code used for generating the examples in the paper is contained in the Python library \emph{trilearn} available at \url{https://github.com/felixleopoldo/trilearn}.


\label{sec:introduction}
% section introduction (end)

==> introduction.tex <==
Decomposable graphs and their junction-tree representations as auxiliary data structure have been used in various contexts; examples include computational geometry, large-scale estimation of random graph models with local dependence, statistical inference, such as sparse covariance and concentration matrix computation, contingency table analysis, and probabilistic graphical models.\jimmy{Add references for all these applications.} 

%[Motivation of the proposed junction-tree sampler:  the  graph  itself  is one of unknowns in the model and sampling technique is needed.] 


%The application that motivated the development of this paper
%is Bayesian structure learning in probabilistic graphical models. 
%In this context, the vertices of the graph represent random variables and the edge set encodes the dependence structure of a multivariate probability distribution.  


%where the junction tree itself is the state variable. The probability of one specific junction tree in this formulation is defined as the underlying graph probability scaled by the number of equivalent junction tree representations. 
%It is shown in  \citet{doi:10.1198/jcgs.2009.07129} that the computational complexity of the elementary operations required for calculating this number grows as $\mathcal O(p^2)$, where $p$ is the number of vertices in the underlying graph.


The increased interest in decomposable graphs for representing dependence structures in probabilistic graphical models has given rise to several strategies to explore this space using \emph{Monte Carlo} sampling.\jimmy{``Explore''? Maybe something like: ``In the Bayesian setting, structure learning in such models amounts to calculate a posterior distribution defined on the space of decomposable graphs. This has lead to an increasing interest in the development of Monte Carlo methods sampling from possibly very complex distributions defined on such spaces.''}
 %sample from distributions over decomposable graphs and junction trees.
%sampling from distributions defined over the space of decomposable graphs is achieved by \emph{\mcmc} strategies generating trajectories of graphs which are expected to converge to the target distribution.
Such strategies are typically based on variations of the \emph{Metropolis-Hastings algorithm}, where in each step, a new graph is proposed on the basis of the previous one by means of edge perturbations.
The proposed graphs are then accepted with probabilities guaranteeing reversibility of the resulting Markov kernel.\jimmy{``The proposed graphs \ldots'': I think that we can remove this sentence, as the MH algorithm is now considered classical.}
The set of possible moves obtained by single edge perturbations defines a decomposable neighborhood from which new graphs can be sampled; see \emph{e.g}. \citep{frydenberg1989decomposition,Giudici01121999} and \citep{Thomas:2009aa}.\jimmy{Perhaps ``neighborhood in the decomposable-graph space''?}
%By exploiting the junction-tree representation, this neighborhood can be generated explicitly instead of testing decomposability for blindly proposed graphs using for example maximal cardinality search \citep{tarjan1984simple} as proposed in, \emph{e.g.}, \citep{10.2307/2673658,madigan1995graphicalmodels}
\citet{Green01032013} present an \emph{\mcmc}\, (\mcmcabbr)\, sampling scheme targeting a given probability mass function over the space of decomposable graphs through an extended version defined over the space of junction trees. 
In this formulation, the value of the extended probability mass function for a given junction tree is given by the probability of the underlying graph divided by the number of junction-tree representations of that graph.

In this paper, we present two new algorithms for manipulating and sampling junction trees, which we call the \emph{\jte} (or the \emph{Christmas-tree algorithm}) and the \emph{\jtc}. % for sequentially sampling of junction trees.
The \jteabbr\, (\jtcabbr) expands (collapses) a junction tree by randomly adding (removing) one vertex to (from) the underlying decomposable graph.
These algorithms are complementary in the sense that any junction tree collapsed by the \jtcabbr\, could be sampled with positive probability by the \jte, and vice versa.
% In this paper, we present a new algorithm which we call the \emph{\jte} or the  \emph{Christmas-tree algorithm}, for sequential sampling of junction trees.
% the algorithm we propose constructs incrementally junction trees by expanding randomly the underlying decomposable graph one vertex at a time.
%It differs substantially from the above-mentioned methods; rather than perturbing the edge set for a fixed set of vertices, the algorithm we propose constructs incrementally junction trees by expanding randomly the underlying decomposable graph one vertex at a time.
%The relevance of our suggested algorithm is justified from a Bayesian structure learning perspective, where it opens for a  novel, sequential approach for approximating \emph{weakly structural Markov} distributions \citep{green2017structural} over decomposable graphs based on \smc.
%In this setting the \jteabbr\, is employed as proposal kernel.
% sequential Monte Carlo (SMC) perspective for approximating \emph{weakly structural Markov} distributions over decomposable graphs; see \citep{green2017structural}, where the  \jteabbr\, is employed as proposal kernel.
Two specific theoretical properties possessed by the \jteabbr\, are of crucial importance.
%in this application.
The first one is the ability to generate any junction tree with a given number of vertices in its decomposable graph.
The second is that the transition probabilities of the kernel can be computed efficiently. 


% motivate why junction tree space
We demonstrate that both algorithms together can be employed to construct a \smc\, (\smcabbr) sampler for approximating arbitrary distributions  over decomposable graphs, using the temporalisation technique from \cite{olsson2019}.
Specifically, the \jtc\, is used to extend the junction tree distribution to a path space and the \jte\, is used as proposal kernel on this new space of junction trees of increasing dimension.

Our proposed sampling techniques provides deeper insights into cardinalities of both spaces of junction trees and underlying decomposable graphs, and how they relate to each other. 
Using the \smcabbr\, sampler, we derive and provide unbiased estimates for the number of decomposable graph and junction trees with any given number of vertices. 
This importance-sampling approach to the combinatorics of decomposable graphs an junction trees is the first of its kind.
\citet{countchordal} provides a closed form expression for the number of decomposable graphs, however calculations are only tractable for a very limited number of vertices.
Up to our knowledge, there is no closed for expression for the number of junction trees.

% By using the \jtc to create an extended target distribution, we demonstrate that the \jte can be used as a proposal kernel in a \smcabbr\, 
% sampling approach, we are able to provide unbiased estimates of normalising constants for weakly structural Markov laws.
%[Change: 
%\citet{olsson2019} show that, by incorporating the \smcabbr\, sampler in a \emph{particle Gibbs} sampler, it is possible to provide \emph{global moves} on the decomposable graph space, in contrast to local edge perturbations.
%As a consequence the mixing properties of the resulting Markov chain are substantially improved.
%A thorough presentation of the \smcabbr\, algorithm together with the particle Gibbs sampling  scheme and further applications to  Bayesian structure learning  are presented in %the companion papers
%\citep{olsson2019, graphpred}. ]

%[In the area of probabilistic graphical models, where graphs are used to describe the dependence structure of a multivariate probability distribution, a family of distributions which are Markov with respect to a decomposable graph is typically called a \emph{decomposable graphical model}, \cite{lauritzen1996}.
%Such models have a particularly appealing property that their distributions factorises as local distributions of the cliques and separators, which makes inference tasks in these models directly removes the problem of unknown normalising constants as is the problem with ordinary undirected graphs. 
%Recent advances \citep{bornn2011bayesian,green2017structural} shows that a certain class of graph distributions over \(\graphsp[\jtind]\), termed \emph{weakly structural Markov}, factorize over the cliques and separators in a similar manner as \emph{decomposable graphical models}.
%Such distributions arise naturally in Bayesian statistics and structure learning as %prior-, and due to their conjugate property, posterior graph distributions. 
%\cite{olsson2019} shows how the junction tree expander and collapser are used in a %particle Gibbs scheme tailored to approximate such distributions efficiently.]


%As a by-product of 
The \jte,\ is related to other approaches of generating junction trees. For example, an algorithm for generation of junction trees presented in \citep{randchord} has similarities to ours in the sense that it incrementally expands the underlying graph in each step of the algorithm.
However, unlike our proposed \jteabbr, this algorithm is restricted to connected decomposable graphs and transition probabilities are not directly provided. 
Further pertinent approaches include \emph{e.g.} \citep{stingo2015efficient}, where focus is Gaussian graphical models which enable faster edge moves by dynamically updating the \emph{perfect sequence} of the cliques in the graph. 

A completely different strategy for decomposable graph sampling based on  {\it tree-dependent bipartiet graphs} is presented in \citet{elmasri2017decomposable, elmasri2017sub}.
\citet{olsson2019} show that, by incorporating the \smcabbr\, sampler in a \emph{particle Gibbs} sampler, it is possible to provide \emph{global moves} on the decomposable graph space, in contrast to local edge perturbations.
%As a consequence the mixing properties of the resulting Markov chain are substantially improved.
%A thorough presentation of the \smcabbr\, algorithm together with the particle Gibbs sampling  scheme and further applications to  Bayesian structure learning  are presented in %the companion papers
%\citep{olsson2019, graphpred}. 





The rest of this paper is structured as follows. Section \ref{sec:preliminaries} introduces some graph notation and a short background on decomposable graphs and the junction tree concept. 
For a more detailed presentation, the reader is referred to \emph{e.g.} \citep{ChordalGraphs} or \citep{lauritzen1996}.
Section~\ref{sec:expanding_a_junction_tree} and Section~\ref{sub:rcta} present the \jteabbr\, and  the \jtcabbr, respectively, along with their corresponding transition probabilities.
Section~\ref{sec:update_mu} provides a novel factorisation of the number of junction trees of a decomposable graph, and demonstrates its computational advantage.
The application of the \jteabbr\, and the \jtcabbr\, in the \smcabbr\, sampling scheme is found in Section~\ref{sec:smc}.
Section~\ref{sec:simulations} provides the numerical study on the combinatorics of decomposable graphs and junction trees.
%the first devoted to 
%Bayesian structure learning in Gaussian decomposable models and the second to decomposable graph combinatorics. 
%In the latter example, \smcabbr\, is used for providing unbiased estimates of the number of decomposable graphs of different number of vertices.
Appendix \ref{appendix:a} is devoted to detailed algorithm descriptions along with the proofs of lemmas and theorems stated in the paper, whereas Appendix \ref{appendix:b} provides an algorithm for randomly connecting a forest into a tree, originally presented in \citep{doi:10.1198/jcgs.2009.07129}.

The  code used for generating the examples in this paper is contained in the Python library \emph{trilearn} available at \url{https://github.com/felixleopoldo/trilearn}.


\label{sec:introduction}
% section introduction (end)


==> simulations.tex <==
% -*- root: opr2018.tex -*-%

We demonstrate two applications of Algorithm~\ref{alg:SMC:update} for estimating the cardinalities of the spaces of decomposable graphs and junction trees, \(|\graphsp[\jtind]|\) and \(|\trsp[\jtind]|\), respectively.

\subsection{Estimating  $|\graphsp[\jtind]|$ } \label{sec:estdec}
There is an exact expression of $|\graphsp[\jtind]|$ presented in \citep{countchordal}, which has been calculated for $\jtind \le 13$.
Another exact algorithm which calculates for \(\jtind\le10\) is proposed in \citep{kawahara2018enumerating}.
An  asymptotic expression for  \(|\graphsp[\jtind]|\)  is  derived in \citep{countchordal} as \(\sum_{l=1}^{\jtind}{\jtind \choose l} 2^{l(\jtind-l)}\).

% Even though the restriction to decomposable graphs is a serious reduction of the graph space, the space is still immense. 

%In this example we provide unbiased estimates of $|\graphsp[\p]|$ and compare them to the space of all undirected graphs with the same number of vertices using \smcabbr. 

%and by considering the SMC scheme for approximating $\graphtarg =\unif[{\graphsp[\jtind]}]$.
In this study on the other hand, we consider Algorithm~\ref{alg:SMC:update} in order to estimate of $|\graphsp[\p]|$ using the target distribution
\begin{align*}
\targ{m}(\tree_{m}) \eqdef \frac{1}{|\graphsp[m]|} \times \frac{1}{\mu(\trgr(\tree_m))}, %\propto \frac{1}{\mu(\trgr(\tree_m))}.
\end{align*}
where \(\tree_{\jtind}\in \trsp[\jtind]\).
With this formulation, an unbiased estimate 
is obtained directly using the estimator \eqref{eq:constest}.
Note that in this setting Line~\ref{smc:updateweight} of Algorithm~\ref{alg:SMC:update} reduces to
\begin{align}
    \frac{ \untarg{m+1}(\tree_{\jtind+1})}{\untarg{\jtind}(\tree_{m})} = \frac{\mu(\trgr(\tree_{m}))}{\mu(\trgr(\tree_{m+1}))},
\end{align}
where \(\tree_{\jtind}\in \trsp[\jtind]\), \(\tree_{\jtind+1}\in \trsp[\jtind+1]\),
for which, as demonstrated by Example~\ref{ex:updatemu}, the computational burden can be substantially reduced by using the factorisation \eqref{eq:mufac} since  \(\tree_{\jtind+1}\in \supp (\prop{\jtind}(\tree_\jtind, \cdot))\).

Table~\ref{tab:numpropdec} shows means and standard errors from 10 
  estimates \(\widehat{|\graphsp[\jtind]|}\)  for $\jtind \in \nn[15]$.
The upper panel of the table shows  $\widehat{|\graphsp[\jtind]|}$ while the lower panel shows $\widehat{|\graphsp[\jtind]|}/2^{{\jtind(\jtind-1)/ 2}}$, i.e. estimates of the fraction of undirected graphs which are decomposable.
For $\jtind\le 13$ the exact enumerations are given in the second column. 
To obtain the estimate with minimal empirical variance, we ran the  \smcabbr\, sampler on the grid of tuning parameters \((\subtreecont,\subtreenonempty) \in [0.3,0.5,0.8]^2\) and found the optimal combination as $\subtreecont=0.5$ and $\subtreenonempty=0.5$. 
The number of particles was set to $\N=10000$.
Figure~\ref{fig:asymtpotics} displays the asymptotic behavior of $|\graphsp[\jtind]|$ and \( \widehat{|\graphsp[\jtind]|}\) for $\jtind\le50$, along with the exact values for $\jtind \leq 13$, justifying a concordance with the exact results.
Each of the 10 estimates took about 10 minutes to calculate.
%Note that the latter two are almost indistinguishable.
\begin{table}[ht!]
\centering
\begin{tabular}{lllll}
$\p $ &\(|\graphsp[\jtind]|\)  &\(\widehat{|\graphsp[\jtind]|}\) & std. err. \\
\hline

4       &       61        &       60.4        &       0.40& \\

5       &       822        &       815        &       16.2 & \\

6       &       1.82        &       1.78        &       0.37 &$\times  10^4 $\\

7       &       6.18        &       5.92        &       0.15 & $\times 10^5$\\

8       &       3.09        &       3.00        &       0.13 & $\times 10^7$\\

9       &       2.19        &       2.14        &       0.09 & $\times 10^9$\\

10      &       2.15        &       2.11        &       0.10 &$\times  10^{11}$\\

11      &       2.88        &       2.80        &       0.18 &$\times  10^{13}$\\

12      &       5.17        &       5.15        &       0.51 & $\times 10^{15}$\\

13      &       1.23        &       1.21        &       0.17 & $\times 10^{18}$\\

14      &       -        &       3.74        &          0.62 &$\times  10^{20}$ \\

15      &       -        &       1.53        &          0.30 & $\times 10^{23}$\\

&&&\\
$\p $ & $|\graphsp[\p]|/2^{{\p(\p-1)/ 2}}$  &$\widehat{|\graphsp[\p]|}/2^{{\p(\p-1)/ 2}}$ & std. err. & \\
\hline

4       &       9.53        &       9.44        &       0.06 & $\times 10^{-1}$\\

5       &       8.03        &       7.96        &       0.16 & $\times 10^{-1}$\\

6       &       5.54        &       5.43        &       0.11 & $\times 10^{-1}$\\

7       &       2.95        &       2.82        &       0.07 & $\times 10^{-1}$\\

8       &       1.15        &       1.12        &       0.05 & $\times 10^{-1}$\\

9       &       3.19        &       3.11        &       0.13 & $\times 10^{-2}$\\

10      &       6.12        &       5.99        &       0.28 & $\times 10^{-3}$\\

11      &       7.99        &       7.78        &       0.51 & $\times 10^{-4}$\\

12      &       7.00        &       6.98        &       0.70 & $\times 10^{-5}$\\

13      &       4.09        &       3.99        &       0.55 & $\times 10^{-6}$\\

14      &       -        &       1.51        &       0.25 & $\times 10^{-7}$\\

15      &       -        &       3.77        &       0.74 & $\times 10^{-9}$\\

 \end{tabular}
\vspace{0.6cm}
%\caption{SMC estimation of the number and the fraction of graphs that are decomposable for $\p\le15$. 


%The number of particles were set to $N=10000$ and the CTA parameters where set to $\subtreecont=0.5, \subtreenonempty=0.8$. 
%The estimated means and standard errors were calculated from $T=50$ independent SMC runs.}
\caption{Sequential Monte Carlo estimation of the number decomposable graphs and the fraction of graphs which are decomposable.}
\label{tab:numpropdec}
\end{table}

\subsection{Estimating  $|\trsp[\jtind]|$ }

%In this example, we estimate \(|\trsp[m]|\) using Algorithm~\ref{alg:SMC:update}.
Up our knowledge there is no known method to efficiently calculate  \(|\trsp[\jtind]|\eqdef\sum_{\graph\in \graphsp[\jtind]}\mu(\graph)\) available in the literature.
However, for \(\jtind \le 5\) it is computationally tractable to first find all the 822 graphs \(\graphsp[\jtind]\) by Monte Carlo sampling and then evaluate \(\mu\) for each of them.%  the exact number may be counted by the sum of for each graph \(\graph \in \graphsp[m]\), where the graphs \( \graphsp[\jtind] \) 
%may be explored by Monte Carlo sampling. 
%This approach was however only computationally tractable for \(\jtind \le 5\).
%However, exact numbers may be counted for \(\jtind \le 5\) by the sum of \(\mu(\graph)\) for each graph \(\graph \in \graphsp[m]\).
%Again, since \(\graphsp[m]\) grows very fast, this method was only tractable for \(\jtind \le 5\).

Similarly with Section~\ref{sec:estdec} we find an unbiased estimator for  \(|\trsp[\jtind]|\) by constructing a target distribution $\targ{m}$ as
\begin{align*}
\targ{m}(\tree_{m}) \eqdef \frac{1}{|\trsp[m]|},% \propto 1.
\end{align*}
where \(\tree_{\jtind}\in \trsp[\jtind]\) and use \eqref{eq:constest}.
%Thus an unbiased estimator of \(|\trsp[\jtind]|\) is provided by \eqref{eq:constest}.
Note that with this setting the first factor in Line~\ref{smc:updateweight} of Algorithm~\ref{alg:SMC:update} simplifies as
\begin{align}
    \frac{ \untarg{m+1}(\tree_{\jtind+1})}{\untarg{\jtind}(\tree_{m})} = 1, %\1_{\trsp[\jtind+1]}(\tree[\jtind+1]).
\end{align}
for any \(\tree_{\jtind}\in \trsp[\jtind]\), \(\tree_{\jtind+1}\in \supp (\prop{\jtind}(\tree_\jtind, \cdot))\).
(Det här ser lite skumt ut, vilken indikatorfunktion menade du att jag skulle använda här, Jimmy? \(\1_{\trsp[\jtind+1]}\)? )

The third and fourth column of the upper panel in Table~\ref{tab:numtrees} shows estimated mean and standard deviation of \(\widehat{|\trsp[\jtind]|}\) for \(\jtind\le 15 \) taken over 10 estimates. 
The true values for are shown in the first column for \(\jtind\le 5\).

The lower panel of Table~\ref{tab:numtrees} considers the average number of junction trees per decomposable graph with a given number of nodes, \(|\trsp[\p]|/|\graphsp[\p]|\).
True number as are shown in the first column, and the estimated mean and standard deviation of the quantity \(\widehat{|\trsp[\p]|}/\widehat{|\graphsp[\p]|}\) are shown in the third and fourth column. 
Interestingly, Figure~\ref{fig:treespergraph} indicates an exponential growth rate of the estimated junction trees per decomposable graph for \(\p\le 50\).
Each of the 10 estimates took about 6 minutes to finish.
\begin{table}[ht!]
\centering
\begin{tabular}{lllll}
$\p $ &\(|\trsp[\p]|\)  &\(\widehat{|\trsp[\p]|}\) & std. err. \\
\hline


1       &       1        &       1        &       0.00        &       \\

2       &       2        &       2        &       0.00        &       \\

3       &       10        &       10        &       0.03        &      \\

4       &       108        &       106        &       1.41        &      \\

5       &       2.09        &       2.03        &       0.03        &       $\times 10^{3}$ \\

6       &       -        &       6.10        &       0.10        &       $\times 10^{4}$ \\

7       &       -        &       2.76        &       0.08        &       $\times 10^{6}$ \\

8       &       -        &       1.79        &       0.07        &       $\times 10^{8}$ \\

9       &       -        &       1.63        &       0.11        &       $\times 10^{10}$ \\

10      &       -        &       2.00        &       0.18        &       $\times 10^{12}$ \\

11      &       -        &       3.37        &       0.32        &       $\times 10^{14}$ \\

12      &       -        &       7.45        &       0.88        &       $\times 10^{16}$ \\

13      &       -        &       2.12        &       0.30        &       $\times 10^{19}$ \\

14      &       -        &       7.87        &       1.34        &       $\times 10^{21}$ \\

15      &       -        &       3.88        &       0.80        &       $\times 10^{24}$ \\
&&&\\
$\p $ & $|\trsp[\p]|/|\graphsp[\p]|$  &$\widehat{|\trsp[\p]|}/ \widehat{|\graphsp[\p]|}$ & std. err.  \\
\hline

1       &       1        &       1        &       0.00 \\

2       &       1        &       1        &       0.00 \\

3       &       1.25        &       1.25&       0.00 \\

4       &       1.77        &       1.76        &       0.03 \\

5       &       2.54        &       2.49        &       0.07 \\

6       &       -        &       3.43        &       0.1 \\

7       &       -        &       4.66        &       0.23 \\

8       &       -        &       5.99        &       0.45 \\

9       &       -        &       7.67        &       0.64 \\

10      &       -        &       9.51        &       0.90 \\

11      &       -        &       12.1        &       1.35 \\

12      &       -        &       14.6        &       1.98 \\

13      &       -        &       17.9        &       3.11 \\

14      &       -        &       21.5        &       4.23 \\

15      &       -        &       26.1        &       6.16 \\

 \end{tabular}
\vspace{0.6cm}
%\caption{SMC estimation of the number and the fraction of graphs that are decomposable for $\p\le15$. 


%The number of particles were set to $N=10000$ and the CTA parameters where set to $\subtreecont=0.5, \subtreenonempty=0.8$. 
%The estimated means and standard errors were calculated from $T=50$ independent SMC runs.}
\caption{Sequential Monte Carlo estimation of the number junction trees and the expected number of junction trees per decomposable graph.}
\label{tab:numtrees}
\end{table}

\begin{figure}[!ht]%[htbp]
    \centering
    \includegraphics[width=0.6\textwidth]{{figures/nchordal.eps}}
    \caption{The number of decomposable graphs as a function of the number of vertices.}
    \label{fig:asymtpotics}
\end{figure}

\begin{figure}[!ht]%[htbp]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/output.png}
    \caption{Estimates of the expected number of junction trees per decomposable graph.}
    \label{fig:treespergraph}
\end{figure}
% \subsection{Estimating the clique number} % (fold)
% \label{sub:estimating_the_clique_number}

% In this example, we estimate the \emph{clique number} (number of nodes in the largest clique) distribution induced by $\unif[{\graphsp[\p]}]$.
% Using the same parameter settings, Figure~\ref{fig:cliquenumber_histogram} displays 10 SMC estimates of the distribution where \(\p=15\).
% The black bars at the top of each staple indicate the standard error of the corresponding estimate.
% Notably, from a prior specification perspective, most of the probability mass is concentrated around the values 5, 6, and 7, meaning that the uniform prior in this case gives strong preference for these clique numbers. 



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/clique_number_dist_p15_N_10000_T_10}
%     \caption{Empirical clique number distributions averaged over $10$ SMC estimates.}
%     \label{fig:cliquenumber_histogram}
% \end{figure}

==> smc.tex <==
% -*- root: opr2018.tex -*-
We demonstrate how the \jteabbr\, and the \jtcabbr\, can be cast into the framework of \smcabbr\, setting for sampling from an arbitrary distribution \(\targ{\jtind}\) defined on \(\trsp[\jtind]\).
Following the \emph{temporalisation} procedure presented in \citep{olsson2019}, we consider the extended path space \(\trsp[1:\jtind]\eqdef\trsp[1]\times \dots \times \trsp[\jtind] \) and
let the target distribution on this space be defined as
\begin{align} \label{eq:norm_embeded}
\targpath{m}(\tree_{1:m}) &
\eqdef
\prod_{\ell=1}^{m-1}\frac{\targ{\ell+1}(\tree_{\ell+1})}{\targ{\ell}(\tree_{\ell})}\times \bk{\ell}(\tree_{\ell+1},\tree_{\ell}),
\end{align}
where \(\tree_{1:\jtind} \in \trsp[1:\jtind]\).
The crucial property of \eqref{eq:norm_embeded} is that the marginal distribution of \(\targpath{m}\) with respect to the \(m\)'th component is exactly \(\targ{m}\).
We leave the details of the justification of \eqref{eq:norm_embeded} to \citep{olsson2019}.

We may sample from \eqref{eq:norm_embeded} using importance sampling with the following proposal distribution, obtained as the product of junction tree expanders
\begin{align} \label{eq:proppath}
\bar q_\jtind(\tree_{1:\jtind})& 
\eqdef 
\prod_{\ell=1}^{\jtind-1}\prop{\ell}(\tree_\ell, \tree_{\ell+1}),
\end{align}
where \(\tree_{1:\jtind} \in \trsp[1:\jtind]\).
%Note that, Theorem \ref{thm:characterization} guarantees that the \eqref{eq:proppath} has support on \(\trsp[\jtind]\).
Note that since Theorem~\ref{thm:rcta} 
%\(\supp(\bk{\ell}(\tree_{\ell+1},\cdot)) \subseteq \supp (\prop{\ell}(\cdot, \tree_{\ell+1}))\) for any \(\tree_{\ell+1} \in \trsp[\ell+1]\) 
implies that \(\supp(\bk{\ell}(\cdot,\tree_{\ell})) \subseteq \supp (\prop{\ell}(\tree_\ell, \cdot))\) for all \(\ell \in \{1,\dots, \jtind\}\), it is readily checked that \( \supp(\targpath{m}) \subseteq \supp(\bar q_\jtind)\).
This property, along with Theorem~\ref{thm:jt_preservation} and \ref{thm:characterization} implies that \eqref{eq:norm_embeded} can be sampled from sequentially using  \(\{\prop{\ell}\}_{\ell=1}^{\jtind-1}\) as proposal transition kernels.

\subsection*{Particle updating and unbiased estimates of normalising constants}
By assuming, recursively, that we are given a sample
$\{ (\treepart{\ell}{i}, \wgt{\ell}{i}) \}_{i = 1}^\N$ of \emph{particles}, each one being a random draw in $\trsp[\ell]$, with associated importance weights (the $\wgt{\ell}{i}$'s) approximating $\targ{\ell}$ in the sense that for any non-negative functional $h$,% \in \mf{\xfd{m}}$,
\begin{align}
    \label{eq:empmeas}
        \sum_{i=1}^{\N} \partarg{\ell}(\treepart{\ell}{i}) h(\treepart{\ell}{i}) \simeq \sum_{\tree \in\trsp[\ell]} \targ{\ell}(\tree) h(\tree) \quad \mbox{as $\N \rightarrow \infty$,}
\end{align}
where
$$
    \partarg{\ell}(\tree) \eqdef \sum_{i = 1}^\N
    \frac{\wgt{\ell}{i}}{\wgtsum{\ell}} \1_{\treepart{\ell}{i}}(\tree),
$$
 denotes the weighted empirical measure associated with the particle sample and $\wgtsum{\ell} \eqdef \sum_{i = 1}^\N \wgt{\ell}{i}$. 
%An updated particle sample $\{ (\epart{m + 1}{i}, \wgt{m + 1}{i}) \}_{i = 1}^\N$ approximating $\targ{m + 1}$ is obtained from Algorithm~\ref{alg:SMC:update}. At Line~\ref{smc:resample} the particles are re-sampled according to the weights.
%\subsubsection{Particle updating scheme}
%Now, given a set of $\N \in \nset$ input particles with corresponding weights $\{ (\epart{\jtind}{i}, \wgt{\jtind}{i}) \}_{i = 1}^\N$ approximating $\targ{\p}(\trex{1:\jtind })$, 
Then, a one-step updating scheme to obtain particles $\{ (\treepart{\ell+1}{i}, \wgt{\ell+1}{i}) \}_{i = 1}^\N$ approximating $\targ{\ell+1}$ in the sense of \eqref{eq:empmeas} is detailed in Algorithm \ref{alg:SMC:update}.

The initial step of Algorithm~\ref{alg:SMC:update} (Line~\ref{smc:resample}) is an auxiliary step where the input particles are re-sampled according to their corresponding weights in order to avoid degeneracy. 
The \jteabbr\, is used on Line~\ref{smc:drawtree} to draw a new junction tree with the vertex $\gennodea[\ell+1] = \ell+1$.
The weights are then updated on Line~\ref{smc:updateweight}.%, where the Markovian form of \eqref{eq:norm_embeded} and the junction tree collapser appears in the 

As a by-product of the \smcabbr\, sampling approach, an unbiased estimator of  the  constant $\sum_{\tree \in \trsp[\jtind]}\untarg{\jtind}(\tree)h(\tree)$ is obtained as
\begin{align}
 %\frac{1}{\wgtsum{m}}
  \frac{1}{\N^\jtind}  \left( \prod_{\ell = 1}^{\jtind-1} \wgtsum{\ell} \right)
 \sum_{i = 1}^\N \wgt{\jtind}{i} h(\treepart{\jtind}{i}),
\end{align}
where \(\untarg{\jtind}\) is the un-normalised version of \(\targ{\jtind}\).
In particular, by letting $h$ be the indicator function on \(\trsp[\jtind]\),
% defined as
% \begin{align}
%     \1_{\trsp[\p]}(\trex{\p}) = 
%     \begin{cases}
%     	1, &\text{ if } \tree_{\p}\in \trsp[\p]\\
%     	0, &\text{ otherwise},
%     \end{cases}
% \end{align}
an unbiased estimator of the  normalising constant of \(\targ{\jtind}\) is obtained by 
\begin{align}
 \frac{1}{\N^\jtind} \prod_{\ell = 1}^{\jtind} \wgtsum{\ell}.  
 \label{eq:constest}  
\end{align}


% The crucial properties which enable for sequential sampling from \eqref{eq:embeded} using $\{\prop{\jtind}\}_{\jtind=1}^{\p}$ as proposal kernels are guaranteed by Theorems \ref{thm:jt_preservation},\ref{thm:characterization}, and \ref{thm:rcta}.
% The approach of extending non-temporal distributions to a path space in order to allow for sequential sampling was first introduced in \citet{10.2307/3879283}.

%In the next section we demonstrate a number of applications of this algorithm.



%\bigskip
\begin{algorithm}[ht!]
    \KwIn{$\{ (\treepart{\ell}{i}, \wgt{\ell}{i}) \}_{i = 1}^\N$}
    \KwOut{$\{ (\treepart{\ell+1}{i}, \wgt{\ell+1}{i}) \}_{i = 1}^\N$}
         \For{$i \gets 1, \ldots, \N$}{
             draw $\ind{\ell + 1}{i} \sim \disc( \{ \wgt{\ell}{j} \}_{j = 1}^\N)$\; \label{smc:resample}
             %draw \(\combpart{m+1}{i} \sim \combkernel{m}(\combpart{m}{\ind{m + 1}{i}}, \cdot)\)\;\label{smc:drawcomb}
             draw \(\treepart{\ell + 1}{i} \sim  \prop{\ell}(\treepart{\ell}{\ind{\ell + 1}{i}}, \cdot)\)\;\label{smc:drawtree}
             %set $\epart{m + 1}{i} \gets (\combpart{m + 1}{i}, \treepart{m + 1}{i})$\;\label{smc:setpart}
            %  set $\displaystyle \wgt{m + 1}{i} \gets
            %  \frac{ \ungraphtarg(\trgr(\treepart{\jtind+1}{i}))}{ \untrtarg(\trgr(\treepart{m}{\ind{m + 1}{i}}))} \times
            % \frac{\jtcount{\trgr(\treepart{m}{\ind{m + 1}{i}})} }{\jtcount{\trgr(\treepart{m+1}{i}) }} \times
            %  \frac{ \bk{m}(\treepart{m + 1}{i},\treepart{m}{\ind{m + 1}{i}}) }{ \prop{m}(\treepart{m}{\ind{m + 1}{i}} , \treepart{m+1}{i})}$\;\label{smc:updateweight}
              set $\displaystyle \wgt{\ell + 1}{i} \gets
             \frac{ \untarg{\ell+1}(\treepart{\ell+1}{i})}{ \untarg{\ell}(\treepart{m}{\ind{\ell + 1}{i}})}\times
             \frac{ \bk{\ell}(\treepart{\ell + 1}{i},\treepart{\ell}{\ind{\ell + 1}{i}}) }{ \prop{\ell}(\treepart{\ell}{\ind{\ell + 1}{i}} , \treepart{m+1}{i})}$\;\label{smc:updateweight}
             \label{alg:smc:weigthupdt}
         }
     \Return{$\{ (\treepart{\ell+1}{i}, \wgt{\ell+1}{i}) \}_{i = 1}^\N$}
     \vspace{0.6cm}
     \caption{Sequential Monte Carlo update.}
     \label{alg:SMC:update}
\end{algorithm}

 
% is a computational bottleneck of the junction tree representation.
% Even though an efficient $\mathcal O(\p^2)$ algorithm for calculating this number is suggested in \citet{doi:10.1198/jcgs.2009.07129}, a non-dynamic update in every step of the algorithm is very demanding.

